Efficient Strongly Polynomial Algorithms for Quantile Regression

Linear Regression is a seminal technique in statistics and machine learning, where the objective is to build linear predictive models between a response (i.e., dependent) variable and one or more predictor (i.e., independent) variables. In this paper, we revisit the classical technique of Quantile Regression (QR), which is statistically a more robust alternative to the other classical technique of Ordinary Least Square Regression (OLS). However, while there exist efficient algorithms for OLS, almost all of the known results for QR are only weakly polynomial. Towards filling this gap, this paper proposes several efficient strongly polynomial algorithms for QR for various settings. For two dimensional QR, making a connection to the geometric concept of $k$-set, we propose an algorithm with a deterministic worst-case time complexity of $\mathcal{O}(n^{4/3} polylog(n))$ and an expected time complexity of $\mathcal{O}(n^{4/3})$ for the randomized version. We also propose a randomized divide-and-conquer algorithm -- RandomizedQR with an expected time complexity of $\mathcal{O}(n\log^2{(n)})$ for two dimensional QR problem. For the general case with more than two dimensions, our RandomizedQR algorithm has an expected time complexity of $\mathcal{O}(n^{d-1}\log^2{(n)})$.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> sections/discussion.tex <==
\section{Challenges in Higher Dimensions}\label{sec:discussion}
Although our $k$-set based {\em QR} solution is extremely efficient in two dimensions, from a theoretical standpoint the same idea does not readily extend to higher dimensions. Let us consider three dimension first. Here the upper bound on the number of $k$-sets is $O(nk^{1.5})$ \cite{sharir2000improved}.
As $k$ is usually a fixed fraction of $n$ in quantile regression, this becomes $O(n^{2.5})$ for any quantile parameter.
If there existed an algorithm to efficiently (say in time $T$) enumerate all the $k$-sets in three dimensions, then our approach for {\em QR} could leverage this algorithm to run in $O(T + n^{2.5})$ time. For appropriately small $T$, our algorithm could then be theoretically better than {\em IPM} (which takes $\Tilde{O}(n^{3.5}\log{(1/\epsilon)})$ time).
However, we do not know of any such efficient enumeration technique for $k$-sets in three dimensions. The  best known algorithm \cite{andrzejak1999optimization} is that of Artur et al., \cite{andrzejak1999optimization} which has an output-sensitive running time of 
$O(|W|  n^2 LP(d+1, n))$ where $W$ is the set of $k$-sets and $LP(d+1, n)$ is the time taken to solve a linear program of $d+1$ variables and $n$ constraints. When $d=3$, this translates in the worst case to 
$O(n^{2.5}  n^2  n)$ = $O(n^{5.5})$, which is slower than IPM. Thus, the interesting open problem is to design a suitably efficient enumeration algorithm for $k$-sets in three dimensions. 
In four dimensions, the situation gets worse. The upper bound on the number of $k$-set is $O(n^2(k+1)^{2-2/45})$ \cite{matousek2006k}.
For any quantile parameter $k = O(n)$, this upper bound becomes approximately $O(n^4)$, which makes such enumeration-based approaches worse than IPM. 
As the number of $k$-set increases significantly in higher dimensions, any $k$-set enumeration-based solution for {\em QR} is worse than IPM. 


Thus for higher dimensions, from a theoretical standpoint, what is needed is a radically different approach that does not rely on a full enumeration of the $k$-sets (for e.g., perhaps a type of ``binary search'' that can quickly eliminate large portions of the arrangement from further consideration in each iteration). 
Nevertheless, from a practical standpoint, we believe that our \un will be useful
for developing practical gradient descent strategies that can rival or
better the state-of-art interior and exterior point methods for quantile
regression. We defer the investigation of theoretical as well as practical solutions to higher dimensional {\em QR} for future work.

% \textcolor{red}{Gautam: have a pagebreak here. Then ``References'' can be on a fresh page. After that, have a section called ``Appendix''}
